A Large Scale Analysis of Semantic Versioning in NPM

The NPM package repository contains over two million packages and serves tens of billions of downloads per-week. Nearly every single JavaScript application uses the NPM package manager to install packages from the NPM repository. NPM relies on a "semantic versioning" ('semver') scheme to maintain a healthy ecosystem, where bug-fixes are reliably delivered to downstream packages as quickly as possible, while breaking changes require manual intervention by downstream package maintainers. In order to understand how developers use semver, we build a dataset containing every version of every package on NPM and analyze the flow of updates throughout the ecosystem. We build a time-travelling dependency resolver for NPM, which allows us to determine precisely which versions of each dependency would have been resolved at different times. We segment our analysis to allow for a direct analysis of security-relevant updates (those that introduce or patch vulnerabilities) in comparison to the rest of the ecosystem. We find that when developers use semver correctly, critical updates such as security patches can flow quite rapidly to downstream dependencies in the majority of cases (90.09%), but this does not always occur, due to developers' imperfect use of both semver version constraints and semver version number increments. Our findings have implications for developers and researchers alike. We make our infrastructure and dataset publicly available under an open source license.

==> figs_and_tables/apr-10-more-combos/number-results/results.tex <==
% These are results from the R Notebook.
% Run the notebook from top to bottom
\newcommand{\dataNumNPMFailures}{47}

\newcommand{\dataMinMinNPMFailures}{26}

\newcommand{\dataMaxMinNPMFailures}{28}

\newcommand{\dataMinNPMTimesoutsMin}{25}

\newcommand{\dataMinNPMTimesoutsMax}{27}

\newcommand{\dataNumPIPUnsupported}{19}

\newcommand{\dataFractionPIPUnsupported}{1.9\%}

\newcommand{\dataNumCargoUnsupported}{3}

\newcommand{\dataFractionCargoUnsupported}{0.3\%}

\newcommand{\dataNumMinNPMFailNPMOk}{18}

\newcommand{\dataNumMinNPMOkNPMFail}{37}

\newcommand{\dataFractionShrinking}{21\%}

\newcommand{\dataFractionShrinkingMinOldness}{7\%}

\newcommand{\dataFractionNewer}{14\%}

\newcommand{\dataFractionOlder}{5\%}

\newcommand{\dataFractionNewerMinimizingNumDeps}{7\%}

\newcommand{\dataFractionOlderMinimizingNumDeps}{20\%}

\newcommand{\dataFSShrinkageMean}{0.86}

\newcommand{\dataFSShrinkageMedian}{0.96}

\newcommand{\dataFSShrinkageQuartileFirst}{82\%}

\newcommand{\dataMeanSlowdown}{2.6s}

\newcommand{\dataMedianSlowdown}{1.6s}

\newcommand{\dataMaxSlowdown}{329s}

\newcommand{\dataMinSlowdown}{-2.3s}

\newcommand{\dataFirstQuantileSlowdown}{0.8s}

\newcommand{\dataThirdQuantileSlowdown}{2.2s}



==> figs_and_tables/apr-10-more-combos/tables/failures.tex <==
% latex table generated in R 4.1.2 by xtable 1.8-4 package
% Wed Apr 13 22:31:19 2022
\begin{table*}[htbp]
  \begin{center}
    \begin{tabular}{lllllrrrr}
      \toprule 
        &  &   & \multicolumn{2}{c}{Minimization Objectives}  &  & \multicolumn{3}{c}{Failures} \\       \cmidrule{4-5} \cmidrule{7-9} 
        Solver & Consistency & Allow cycles? & Primary & Secondary &  Successes& Unsat & Timeout & Other \\ 
      \midrule
        NPM &  &  &  & & 953 &   0 &   0 &  47 \\ 
        \namenpm{} & npm & Yes & Oldness& \# of Dependencies & 972 &   0 &  27 &   1 \\ 
        \namenpm{} & npm & Yes & \# of Dependencies & Oldness & 972 &   0 &  27 &   1 \\

        % \namenpm{} & npm & Yes & min\_duplicates, min\_oldness & 972 &   0 &  27 &   1 \\ 

        \namenpm{} & npm & Yes & Oldness & Duplicate Packages & 973 &   0 &  26 &   1 \\ 

        % \namenpm{} & npm & Yes & min\_oldness & 974 &   0 &  25 &   1 \\ 

        \namenpm{} & no-dups & Yes & Oldness & \# of Dependencies & 926 &  19 &  54 &   1 \\ 

        % \namenpm{} & no-dups & Yes & min\_num\_deps, min\_oldness & 926 &  19 &  54 &   1 \\ 
        % \namenpm{} & no-dups & Yes & min\_oldness & 926 &  19 &  52 &   3 \\ 

        % \namenpm{} & cargo & Yes & min\_oldness, min\_num\_deps & 942 &   3 &  54 &   1 \\ 

        % \namenpm{} & cargo & Yes & min\_num\_deps, min\_oldness & 943 &   3 &  53 &   1 \\ 
        % \namenpm{} & cargo & Yes & min\_duplicates, min\_oldness & 942 &   3 &  54 &   1 \\ 
        % \namenpm{} & cargo & Yes & min\_oldness, min\_duplicates & 943 &   3 &  53 &   1 \\ 
        % \namenpm{} & cargo & Yes & min\_oldness & 949 &   3 &  46 &   2 \\ 

        \namenpm{} & npm & No & Oldness & \# of Dependencies & 972 &   0 &  27 &   1 \\ 
        % \namenpm{} & cargo & No & min\_oldness, min\_num\_deps & 944 &   3 &  52 &   1 \\ 
        \namenpm{} & no-dups & No & Oldness & \# of Dependencies & 926 &  19 &  54 &   1 \\ 
      \bottomrule
    \end{tabular}
  \end{center}
  \caption{Failures that occur when running NPM and different configurations of \namenpm on the \datasetTopName{} dataset.}
  \label{table:failures}
\end{table*}


==> figs_and_tables/apr-10-more-combos/tables/shrinkage_combos.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Wed Aug 31 16:26:05 2022
\begin{table}[ht]
\centering
\begin{tabular}{lrr}
  \hline
Configuration & \# Shrunk (of 477) & \# Enlarged (of 477) \\ 
  \hline
NPM; min\_num\_deps,min\_oldness &  99 &   1 \\ 
  NPM; min\_duplicates,min\_oldness &  36 &   1 \\ 
  PIP; min\_oldness &  36 &   1 \\ 
  Cargo; min\_oldness &  34 &   1 \\ 
  NPM; min\_oldness,min\_num\_deps &  34 &   2 \\ 
   \hline
\end{tabular}
\end{table}


==> figs_and_tables/federico-vuln-exp/results.tex <==
% These are results from the R Notebook.
\newcommand{\dataCveExpTotalCount}{715}

\newcommand{\dataCveExpSuccessCount}{472}

\newcommand{\dataCveExpMaxNpmBetterCount}{235}

\newcommand{\dataCveExpMaxNpmSameCount}{236}

\newcommand{\dataCveExpMaxNpmWorseCount}{1}

\newcommand{\dataCveExpMeanCveDiff}{14.75}

\newcommand{\dataCveExpSuccessPerc}{66\%}

\newcommand{\dataCveExpMaxNpmBetterTotalPerc}{33\%}

\newcommand{\dataCveExpMaxNpmBetterSuccessPerc}{50\%}

\newcommand{\dataCveExpMaxNpmFixedCompletelyCount}{197}



==> figs_and_tables/macro_figures/figure_optimization.tex <==
\begin{figure*}
\begin{center}

\begin{subfigure}{0.45\textwidth}
    \includegraphics[width=\columnwidth]{figs_and_tables/\whichVulnExperiment/plots/cve-diff-hist.pdf}
    \caption{
        A histogram showing CVSS improvement of packages solved with \namenpm{} (configured to minimize vulnerabilities first) 
        compared to NPM's auditing tool. CVSS decreases with \dataCveExpMaxNpmBetterTotalPerc{} of packages.
    }
    \label{figure:cves_hist}
\end{subfigure}
\quad\quad
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\columnwidth]{figs_and_tables/\whichExperiment/plots/oldness_scatterplot.pdf}
\caption{
    \namenpm is configured to minimize
    oldness and the number of dependencies (in that order).
    Each point represents a package, and those below the line
    have newer dependencies, by the metric in \Cref{section:evaluation-better-solutions}. 
    Overall, \namenpm{} finds newer versions for dependencies.
}
\label{figure:oldness}
\end{subfigure}

\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\columnwidth]{figs_and_tables/\whichExperiment/plots/shrinkage.pdf}
\caption{
    A CDF of the fraction of dependencies compared to NPM, when \namenpm{}
    is configured to
    \begin{inparaenum}[a)]
        \item minimize dependencies then oldness (red CDF), or
        \item minimize oldness then dependencies (blue CDF).
    \end{inparaenum}
    \namenpm can reduce dependencies
    in about \dataFractionShrinking{} of packages.
}
\label{figure:shrinkage}
\end{subfigure}
\quad\quad
\begin{subfigure}{0.45\textwidth}
\includegraphics[width=\columnwidth]{figs_and_tables/\whichExperiment/plots/disk_shrinkage_ecdf.pdf}
\caption{
    A CDF of the ratio of disk space of packages
    solved using \namenpm{} (configured to minimize number of dependencies, then oldness) 
    vs NPM. \namenpm{} can reduce space required.
}
\label{disk_shrinkage}
\end{subfigure}
\end{center}

\caption{
    Comparing NPM's to \namenpm{}'s solution quality. 
    These plots ignore failures in both solvers
    and have \namenpm{} configured to use NPM-style consistency
    and allow cycles.
}
\end{figure*}

==> figs_and_tables/macro_figures/figure_performance.tex <==
\begin{figure}
    \includegraphics[width=\columnwidth]{figs_and_tables/\whichExperiment/plots/slowdown_ecdf_no_outliers.pdf}
    \caption{
        CDFs of the additional time taken by \namenpm{}
        to solve and install packages compared to NPM, ignoring timeouts and failures,
        with outliers ($> 20s$)  excluded.
        The outliers take up to \dataMaxSlowdown{} extra seconds, 
        but the mean and median slowdowns are only 
        \dataMeanSlowdown{} and \dataMedianSlowdown{}, respectively.
        In this experiment \namenpm{} was configured with
        NPM-style consistency, allowing cycles, and minimizing oldness first and
        then number of dependencies.
    }
    \label{figure:slowdown_no_outliers}
\end{figure}



==> figs_and_tables/redo_with_pip_optimization/number-results/results.tex <==
% These are results from the R Notebook.
% Run the notebook from top to bottom
\newcommand{\dataNumNPMFailures}{47}

\newcommand{\dataMinMinNPMFailures}{26}

\newcommand{\dataMaxMinNPMFailures}{28}

\newcommand{\dataMinNPMTimesoutsMin}{25}

\newcommand{\dataMinNPMTimesoutsMax}{27}

\newcommand{\dataNumPIPUnsupported}{35}

\newcommand{\dataFractionPIPUnsupported}{3.5\%}

\newcommand{\dataNumCargoUnsupported}{3}

\newcommand{\dataFractionCargoUnsupported}{0.3\%}

\newcommand{\dataNumMinNPMFailNPMOk}{18}

\newcommand{\dataNumMinNPMOkNPMFail}{37}

\newcommand{\dataFractionShrinking}{21\%}

\newcommand{\dataFractionShrinkingMinOldness}{7\%}



==> figs_and_tables/redo_with_pip_optimization/tables/failures.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Sun Aug 28 21:39:01 2022
\begin{table}[ht]
\centering
\begin{tabular}{llllrrr}
  \hline
Solver & Consistency & DisallowCycles & Minimization & Unsat & Timeout & Other \\ 
  \hline
NPM &  &  &  &   0 &   0 &  47 \\ 
  MinNPM & npm & allow\_cycles & min\_oldness,min\_num\_deps &   0 &  27 &   1 \\ 
  MinNPM & npm & disallow\_cycles & min\_oldness,min\_num\_deps &   0 &  27 &   1 \\ 
  MinNPM & cargo & allow\_cycles & min\_oldness,min\_num\_deps &   3 &  54 &   1 \\ 
  MinNPM & cargo & disallow\_cycles & min\_oldness,min\_num\_deps &   3 &  52 &   1 \\ 
  MinNPM & pip & allow\_cycles & min\_oldness,min\_num\_deps &  40 &   2 &  20 \\ 
  MinNPM & pip & disallow\_cycles & min\_oldness,min\_num\_deps &  42 &  18 &   1 \\ 
  MinNPM & npm & allow\_cycles & min\_num\_deps,min\_oldness &   0 &  27 &   1 \\ 
  MinNPM & cargo & allow\_cycles & min\_num\_deps,min\_oldness &   3 &  53 &   1 \\ 
  MinNPM & pip & allow\_cycles & min\_num\_deps,min\_oldness &  40 &   2 &  20 \\ 
  MinNPM & npm & allow\_cycles & min\_duplicates,min\_oldness &   0 &  27 &   1 \\ 
  MinNPM & cargo & allow\_cycles & min\_duplicates,min\_oldness &   3 &  54 &   1 \\ 
  MinNPM & npm & allow\_cycles & min\_oldness,min\_duplicates &   0 &  26 &   1 \\ 
  MinNPM & cargo & allow\_cycles & min\_oldness,min\_duplicates &   3 &  53 &   1 \\ 
  MinNPM & npm & allow\_cycles & min\_oldness &   0 &  25 &   1 \\ 
  MinNPM & cargo & allow\_cycles & min\_oldness &   3 &  46 &   2 \\ 
  MinNPM & pip & allow\_cycles & min\_oldness &  40 &   2 &  20 \\ 
   \hline
\end{tabular}
\end{table}


==> figs_and_tables/redo_with_pip_optimization/tables/shinkage_combos.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Sun Aug 28 21:39:02 2022
\begin{table}[ht]
\centering
\begin{tabular}{lrr}
  \hline
Configuration & \# Shrunk (of 477) & \# Enlarged (of 477) \\ 
  \hline
NPM; min\_num\_deps,min\_oldness & 100 &   1 \\ 
  NPM; min\_duplicates,min\_oldness &  36 &   1 \\ 
  PIP; min\_oldness &  36 &  34 \\ 
  Cargo; min\_oldness &  34 &   1 \\ 
  NPM; min\_oldness,min\_num\_deps &  34 &   2 \\ 
   \hline
\end{tabular}
\end{table}


==> figs_and_tables/rerun-vuln-exp/results.tex <==
% These are results from the R Notebook.
\newcommand{\dataCveExpTotalCount}{715}

\newcommand{\dataCveExpSuccessCount}{452}

\newcommand{\dataCveExpMaxNpmBetterCount}{42}

\newcommand{\dataCveExpMaxNpmSameCount}{410}

\newcommand{\dataCveExpMaxNpmWorseCount}{0}

\newcommand{\dataCveExpMeanCveDiff}{1.75}

\newcommand{\dataCveExpSuccessPerc}{63\%}

\newcommand{\dataCveExpMaxNpmBetterTotalPerc}{6\%}

\newcommand{\dataCveExpMaxNpmBetterSuccessPerc}{9\%}



==> figs_and_tables/test_results/matrix.tex <==
% This is calculated here:
% https://github.com/donald-pinckney/pacsolve/blob/master/slurm/permanently_saved_results/test_top1000_analysis.ipynb

\def\testRunningMatrix{{
{563,  7},  %row 1
{   38,127},  %row 2
}}

==> related.tex <==
\section{Related Work}
\label{related}

Van der Hoek et al. first discussed the idea of ``software release
management''~\cite{van1997software} for large numbers of independent packages in 1997,
and the first package managers for Linux distributions emerged at around the same
time~\cite{rpm,apt}. The version selection problem was first shown to be NP-complete and
encoded as a SAT and Constraint Programming (CP) problem by Di Cosmo et
al.~\cite{dicosmo:edos,mancinelli+:ase06-foss-distros} in 2005. This early work led to
the Mancoosi project, which developed the idea of a modular package manager with
customizable solvers~\cite{abate2012dependency,abate-2013-modular-package-manager}. This
work centers around the Common Upgradeability Description Format (CUDF), an input format
that can be generated by package manager front-ends to describe a given upgradeability
scenario to a back-end solver.

CUDF facilitated the development of solver {\it implementations} using Mixed-Integer
Linear Programming, Boolean Optimization, and Answer Set
Programming~\cite{michel+:lococo2010,argelich+:lococo2010,gebser+:2011-aspcud}, and many
modern Linux distributions have adopted CUDF-like approaches~\cite{abate2020dependency}.
OPIUM~\cite{tucker+:icse07-opium} examined the use of ILP with weights to minimize the
number of bytes downloaded or the total number of packages installed.

While package managers have their roots in Linux distributions, they have evolved
considerably since the early days. Modern language ecosystems have evolved their own
package managers~\cite{npm,pip,cargo,weizenbaum:pubgrub18}, with solver requirements
distinct from those of a traditional Linux distribution. Distribution package managers
typically manage only a single, global installation of each package, while language
package managers are geared more towards programmers and allow {\it multiple}
installations of the same software package.

For the most part, language ecosystems have avoided using complete solvers.
There are a number of reasons for this. Solvers are complex, and they have a
steep learning curve. Even on the Linux distribution side, so-called
\emph{functional} Linux distributions~\cite{dolstra+:lisa04,courtes-guix-2015}
eschew solving altogether, opting instead to focus on reproducibile
configurations maintained by humans. Most programmers do not know how to use
solvers effectively, and fast, high-quality solver implementations do not exist
for new and especially interpreted languages. Moreover, package managers are now
fundamental to software ecosystems, and most language communities prefer to
write and maintain their core tooling in their own langage.

Despite this, developers are starting to realize the need for completeness and
well defined dependency resolution semantics~\cite{abate2020dependency}. The
Python community, plagued by inconsistencies in resolutions done by PIP
has recently switched to a new resolver with a proper
solver~\cite{pip-new-resolver}. Dart now uses a custom CDCL SAT solver called
{\tt PubGrub}~\cite{weizenbaum:pubgrub18}, and Rust's Cargo~\cite{cargo} package
manager is moving towards this approach~\cite{pubgrub-rs}.
However, these solvers use ad-hoc techniques baked into the implementations
to produce desirable solutions, such as exploring package versions sorted by version number.
These are not guaranteed to be optimal, and it is unclear how to add or modify objectives to these types of solvers.
In contrast, \namebackend{} allows for a declarative specification
of multiple prioritized optimization objectives


Solvers themselves are becoming more accessible through tools like
Rosette~\cite{torlak2013growing}, which makes features of the
Z3~\cite{demoura+:tacas08} SMT solver accessible within regular
Racket~\cite{felleisen2015racket} code. Spack~\cite{gamblin+:sc15} makes complex
constraints available in a Python DSL, and implements their semantics using
Answer Set Programming~\cite{gebser+:aicomm11,gamblin:fosdem20-concretizer}. APT
is moving towards using Z3 to implement more sophisticated dependency
semantics~\cite{klode:z3-apt}.

The goal of our work is to further separate concerns away from package manager
developers. \namebackend focuses on {\it consistency} criteria and
formalizes the {\it guarantees} that can be offered by package
solvers. NPM~\cite{npm}'s tree-based solver avoids the use of an
NP-complete solver by allowing multiple, potentially {\it inconsistent} versions
of the same package in a tree. Tools like Yarn~\cite{yarn} attempt to
improve on this with post-hoc techniques like {\it
hoisting}~\cite{maier:hoisting} that deduplicate the dependency graph {\it
after} solving. However, they still do not guarantee consistent
semantics. \namebackend{} provides the best of all these worlds. It combines the
flexibility of multi-version resolution algorithms with the guarantees of
complete package solvers, and it guarantees a {\it minimal} dependency graph.


==> tikz_pictures/different_solution_macros.tex <==
\newcommand{\differentFigPA}{\texttt{debug}}
\newcommand{\differentFigAvOne}{\texttt{4.3.4}}

\newcommand{\differentFigPB}{\texttt{ms}}
\newcommand{\differentFigBvOne}{\texttt{1.0.0}}
\newcommand{\differentFigBvTwo}{\texttt{2.1.0}}
\newcommand{\differentFigBvThree}{\texttt{2.1.2}}

\newcommand{\differentFigConstraintA}{*}
\newcommand{\differentFigConstraintApip}{}
\newcommand{\differentFigConstraintB}{< 2.1.2}

==> tikz_pictures/different_solutions.tex <==
\begin{figure}[htbp]
\centering
\begin{subfigure}{0.22\textwidth}
\begin{tikzpicture}[
    node distance=1.7cm,
    every node/.style={circle,draw,align=center,font=\scriptsize}]
    \node(0) {\differentFigPB\\\differentFigBvOne};
    \node[below of=0] {\differentFigPB\\\differentFigBvTwo};
    \node[right of=0](2) {\differentFigPB\\\differentFigBvThree};
    \node[below of=2](1) {\differentFigPA\\\differentFigAvOne};
    \path (1) edge[bend right,->] (2);
\end{tikzpicture}
\caption{Available packages}
\label{all-different-universe}
\end{subfigure}
%
\vline\quad
%
\begin{subfigure}{0.24\textwidth}
\begin{lstlisting}[escapeinside={|}{|}]
"dependencies": {
  "|\differentFigPA|": "|\differentFigConstraintA|",
  "|\differentFigPB|": "|\differentFigConstraintB|"
}
\end{lstlisting}

\begin{tikzpicture}[
    node distance=1.7cm,
    every node/.style={circle,draw,align=center,font=\scriptsize}]
    \node(cxt) {\textit{context}};
    \node[right of=cxt](b1) {\differentFigPB\\\differentFigBvTwo};
    \node[below of=cxt](a) {\differentFigPA\\\differentFigAvOne};
    \node[right of=a](b2) {\differentFigPB\\\differentFigBvThree};
    \path (cxt) edge[bend right,->] (a);
    \path (cxt) edge[bend right,->] (b1);
    \path (a) edge[bend right,->] (b2);
\end{tikzpicture}

\caption{JavaScript/NPM}
\label{all-different-npm}
\end{subfigure}
%
\vline
\quad
%
\begin{subfigure}{0.22\textwidth}
requirements.txt:
\begin{lstlisting}[escapeinside={|}{|}]
|\differentFigPA| |\differentFigConstraintApip|
|\differentFigPB| |\differentFigConstraintB|
\end{lstlisting}

\fbox{\footnotesize{Unsolvable}}
\caption{Python/PIP}
\label{all-different-pip}
\end{subfigure}
%
\vline\quad
%
\begin{subfigure}{0.22\textwidth}
\begin{lstlisting}[escapeinside={|}{|}]
[dependencies]
|\differentFigPA| = "|\differentFigConstraintA|"
|\differentFigPB| = "|\differentFigConstraintB|"
\end{lstlisting}

\begin{tikzpicture}[
    node distance=1.7cm,
    every node/.style={circle,draw,align=center,font=\scriptsize}]
    \node(cxt) {\textit{context}};
    \node[right of=cxt](b1) {\differentFigPB\\\differentFigBvOne};
    \node[below of=cxt](a) {\differentFigPA\\\differentFigAvOne};
    \node[right of=a](b2) {\differentFigPB\\\differentFigBvThree};
    \path (cxt) edge[bend right,->] (a);
    \path (cxt) edge[bend right,->] (b1);
    \path (a) edge[bend right,->] (b2);
\end{tikzpicture}

\caption{Rust/Cargo}
\label{all-different-cargo}
\end{subfigure}


\caption{
    The \differentFigPA{} package (a debug logging library) and \differentFigPB{} package (a library to convert times values to miliseconds) 
    are available on \url{npmjs.com}, with 16.4 billion and 12.6 billion total downloads, respectively. 
    \cref{all-different-universe} shows a subset of the versions of each package, and \differentFigPA{}'s exact version constraint on \differentFigPB{}.
    \cref{all-different-pip,all-different-npm,all-different-cargo} illustrate the three different results generated by NPM, PIP, and Cargo if the programmer
    were to ask for any version of \differentFigPA{} and any version of \differentFigPB{} strictly less than \differentFigBvThree{}, supposing the versions
    shown in \cref{all-different-universe} are all the versions in the universe.
}
\label{all-different-fig}
\end{figure}

==> tikz_pictures/rosette.tex <==
% Define the layers to draw the diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% Define block styles used later

\tikzstyle{node}=[draw, fill=blue!20, text width=6em,
     minimum height=2.5em,drop shadow]
\tikzstyle{attribute}=[draw, fill=green!20, %text width=em,
    text centered, %minimum height=2.5em,
    drop shadow, rounded corners]
\tikzstyle{root}=[draw, fill=red!20, text width=5em,
    text centered, minimum height=2.5em,drop shadow,rounded corners]

\tikzstyle{concreteEdge} = [draw, -{Latex[length=3mm,width=3mm]}, line width=0.3mm]
\tikzstyle{symbolicEdge} = [draw, -{Latex[length=2mm,width=2mm]}, line width=0.2mm, dashed]


\begin{figure}
  \centering
  \begin{tikzpicture}
    \node (a101) [node] {\texttt{\differentFigPA{} \differentFigAvOne{}}};
    \path (a101.east)+(-0.2,+0.45) node (a101inc) [attribute] {$\mathit{included}$};
    \path (a101.east)+(0.1,-0.45) node (a101depth) [attribute] {$\mathit{depth}$};
    \path (a101.south west)+(0.2,0.0) node (a101Port) {};
    % \fill (a101Port) circle (0.1cm);
    \path (a101.east)+(-0.1, 0) node (a101Out) {};
    % \fill (a101Out) circle (0.1cm);

    \begin{pgfonlayer}{background}
      \path (a101.west |- a101.north)+(-0.3,0.45) node (a) {};
      \path (a101.west |- a101.south)+(-0.3,-0.95) node (b) {};
      \path (a101.south -| a101inc.east)+(+0.3,-0.95) node (c) {};

      \path[fill=yellow!20,rounded corners, draw=black!50, dashed]
          (a) rectangle (c);
      \path (a101.south)+(0.5,-0.65) node {Package \differentFigPA};
      % \path (asr1.north west)+(-0.2,0.2) node (a) {};
    \end{pgfonlayer}

    \path (b)+(0.5, 0) node (aPort) {};
    \fill (aPort) circle (0.1cm);



    \path (a101.east)+(3.4,0) node (b101) [node] {\texttt{\differentFigPB{} \differentFigBvOne{}}};
    \path (b101.east)+(0.3,+0.3) node (b101inc) [attribute] {$\mathit{included}$};
    \path (b101.east)+(0.3,-0.3) node (b101depth) [attribute] {$\mathit{depth}$};
    \path (b101.west)+(0.1,0) node (b101Port) {};
    % \fill (b101Port) circle (0.1cm);

    \path (b101.south)+(0.0,-1.0) node (b201) [node] {\texttt{\differentFigPB{} \differentFigBvTwo{}}};
    \path (b201.east)+(0.3,+0.3) node (b201inc) [attribute] {$\mathit{included}$};
    \path (b201.east)+(0.3,-0.3) node (b201depth) [attribute] {$\mathit{depth}$};
    \path (b201.west)+(0.1,0) node (b201Port) {};
    % \fill (b201Port) circle (0.1cm);

    \path (b201.south)+(0.0,-1.0) node (b202) [node] {\texttt{\differentFigPB{} \differentFigBvThree{}}};
    \path (b202.east)+(0.3,+0.3) node (b202inc) [attribute] {$\mathit{included}$};
    \path (b202.east)+(0.3,-0.3) node (b202depth) [attribute] {$\mathit{depth}$};
    \path (b202.west)+(0.1,0) node (b202Port) {};
    % \fill (b202Port) circle (0.1cm);

    \begin{pgfonlayer}{background}
      \path (b101.west |- b101.north)+(-0.7,0.3) node (a) {};
      \path (b101.west |- b202.south)+(-0.7,-0.8) node (b) {};
      \path (b202.south -| b202inc.east)+(+0.3,-0.8) node (c) {};

      \path[fill=yellow!20,rounded corners, draw=black!50, dashed]
          (a) rectangle (c);
      \path (b202.south)+(0.5,-0.5) node {Package \differentFigPB{}};
      % \path (asr1.north west)+(-0.2,0.2) node (a) {};
    \end{pgfonlayer}

    \path (a) -- node (bPortMid) {} (b);
    \path (bPortMid)+(0,-0.5) node (bPortRoot) {};
    \fill (bPortRoot) circle (0.1cm);
    \path (bPortMid)+(0,0.7) node (bPortA) {};
    \fill (bPortA) circle (0.1cm);


    \path (a101 |- b202) node (root) [root] {Root};
    \path (root.east)+(0.3,+0.45) node (rootinc) [attribute] {$\mathit{included}$};
    \path (root.east)+(0.3,-0.45) node (rootdepth) [attribute] {$\mathit{depth}$};

    \path (root.north)+(0,0) node (rootOut1) {};
    \path (root.east)+(-0.1,0) node (rootOut2) {};

    % \fill (rootOut1) circle (0.1cm);
    % \fill (rootOut2) circle (0.1cm);



    \path [concreteEdge] (rootOut1) edge[bend left] node []{} (aPort);
    \path [concreteEdge] (rootOut2) edge[bend right] node []{} (bPortRoot);
    \path [symbolicEdge] (aPort) edge[bend left] node []{} (a101Port);

    \path [concreteEdge] (a101Out) edge[bend left] node []{} (bPortA);

    \path [symbolicEdge] (bPortRoot) edge[] node []{} (b101Port);
    \path [symbolicEdge] (bPortRoot) edge[] node []{} (b201Port);
    \path [symbolicEdge] (bPortRoot) edge[] node []{} (b202Port);

    \path [symbolicEdge] (bPortA) edge[] node []{} (b101Port);
    \path [symbolicEdge] (bPortA) edge[] node []{} (b201Port);
    \path [symbolicEdge] (bPortA) edge[] node []{} (b202Port);
  \end{tikzpicture}
  \caption{A sample solution graph sketch}
  \label{figure:graph-sketch}
\end{figure}

==> tikz_pictures/test_matrix.tex <==
% Code from: https://tex.stackexchange.com/a/572545

\def\testResultLabels{{"Pass","Fail"}} %class names. Adapt at will
\def\numTestResultLabels{2} %number of classes. Could be automatic, but you can change it for tests.
\def\testRunningMatrixScale{1.5} % 1.5 is a good scale. Values under 1 may need smaller fonts!

\begin{figure}
\begin{center}
\hspace{-40pt}
\begin{tikzpicture}[
    scale = \testRunningMatrixScale,
    %font={\scriptsize}, %for smaller scales, even \tiny may be useful
]

\tikzset{vertical label/.style={rotate=90,anchor=east}}   % usable styles for below
\tikzset{diagonal label/.style={rotate=45,anchor=north east}}

\def\totSamples{0}
\foreach \y in {1,...,\numTestResultLabels}
{
    \foreach \x in {1,...,\numTestResultLabels}
    {
        \pgfmathparse{\testRunningMatrix[\y-1][\x-1]}
        \xdef\totSamples{\totSamples+\pgfmathresult}
    }
}
\pgfmathparse{\totSamples} \xdef\totSamples{\pgfmathresult}  % put the final sum in variable

\foreach \y in {1,...,\numTestResultLabels} %loop vertical starting on top
{
    % Add class name on the left
    \node [anchor=east] at (0.4,-\y) {\pgfmathparse{\testResultLabels[\y-1]}\pgfmathresult}; 
    
    \foreach \x in {1,...,\numTestResultLabels}  %loop horizontal starting on left
    {
    \begin{scope}[shift={(\x,-\y)}]
        \def\mVal{\testRunningMatrix[\y-1][\x-1]} % The value at index y,x (-1 because of zero indexing)
        \pgfmathtruncatemacro{\r}{\mVal}   %
        \pgfmathtruncatemacro{\p}{round(\r/\totSamples*100)}
        \coordinate (C) at (0,0);
        \ifthenelse{\p<50}{\def\txtcol{black}}{\def\txtcol{white}} %decide text color for contrast
        \node[
            draw,                 %draw lines
            text=\txtcol,         %text color (automatic for better contrast)
            align=center,         %align text inside cells (also for wrapping)
            fill=black!\p,        %intensity of fill (can change base color)
            minimum size=\testRunningMatrixScale*10mm,    %cell size to fit the scale and integer dimensions (in cm)
            inner sep=0,          %remove all inner gaps to save space in small scales
            ] (C) {\r\\\p\%};     %text to put in cell (adapt at will)
        %Now if last vertical class add its label at the bottom
        \ifthenelse{\y=\numTestResultLabels}{
        \node [] at ($(C)-(0,0.75)$) % can use vertical or diagonal label as option
        {\pgfmathparse{\testResultLabels[\x-1]}\pgfmathresult};}{}
    \end{scope}
    }
}
%Now add x and y labels on suitable coordinates
\coordinate (yaxis) at (-0.4,-0.75);  %must adapt if class labels are wider!
\coordinate (xaxis) at (0.5+\numTestResultLabels/2, -\numTestResultLabels-1.1); %id. for non horizontal labels!
\node [vertical label] at (yaxis) {\namenpm};
\node []               at (xaxis) {NPM};
\end{tikzpicture}
\end{center}

\caption{
    Results of running tests after solving dependencies with NPM and \namenpm{}. In total only 5\% of packages have a failing test with \namenpm{} but not with NPM. 
}
\label{figure:test_result_matrix}
\end{figure}
